Multilingual Denoising Pre-training for Neural Machine Translation

This paper demonstrates that multilingual denoising pre-training produces significant performance gains across a wide variety of machine translation (MT) tasks. We present mBART -- a sequence-to-sequence denoising auto-encoder pre-trained on large-scale monolingual corpora in many languages using the BART objective. mBART is one of the first methods for pre-training a complete sequence-to-sequence model by denoising full texts in multiple languages, while previous approaches have focused only on the encoder, decoder, or reconstructing parts of the text. Pre-training a complete model allows it to be directly fine tuned for supervised (both sentence-level and document-level) and unsupervised machine translation, with no task-specific modifications. We demonstrate that adding mBART initialization produces performance gains in all but the highest-resource settings, including up to 12 BLEU points for low resource MT and over 5 BLEU points for many document-level and unsupervised models. We also show it also enables new types of transfer to language pairs with no bi-text or that were not in the pre-training corpus, and present extensive analysis of which factors contribute the most to effective pre-training.

==> 01-intro-old.tex <==
\section{Introduction}
\label{sec:intro}
% what is the problem
Self-supervised learning based pre-training~\cite{devlin2018bert,liu2019roberta, yang2019xlnet} has been successfully applied to natural language classification~\cite{wang2019glue}, question answering~\cite{rajpurkar2016squad, eli5}, text generation~\cite{cnn, xsum}, and cross-lingual natural language inference~\cite{conneau2018xnli} tasks. However, limited prior work have explored to how pre-training can be beneficial to machine translation (MT) applictions, which are typically . 

% why is it important

%Previous work has primarily focused on two ways to use monolingual data in machine translation: backtranslation and pre-training. Backtranslation approaches use a learned model to create pseudo-bitext that 

%There are two categories of pre-trained models: encoder-only~\cite{devlin2018bert, liu2019roberta, yang2019xlnet} and encoder-decoder~\cite{lewis2019bart, 2019t5, song2019mass}.  
%Work also has been done to extend English pre-trained models to multilingual models~\cite{lample2019cross, conneau2019unsupervised, song2019mass}. The State of The Art results from those works have showed that attention weights can be shared across languages. Different efforts of exploiting pre-training on MT include XLM~\cite{lample2019cross} initializing encoder and decoder by the same encoder-only pre-train, while Mass~\cite{song2019mass} initializing the seq2seq model by its encoder-decoder pre-train. Besides pre-training, another common approach to utilize monolingual corpus is Back Translation (BT), which suffers from building pipeline for each language pair. 

%XLM~\cite{lample2019cross} also demonstrates that training online back translation on an encoder-only pre-trained model initialized encoder of a sequence to sequence system along with an de-noising auto-encoder model initialized decoder can improve unsupervised machine translation tasks.



% technical details
We are here to present a new multilingual pre-training strategy that can be used to initialize encoder-decoder together on multiple machine translation sequence-to-sequence tasks. We train a de-noising auto-encoder sequence to sequence model with Bart~\cite{lewis2019bart} masking strategy on 25 languages monolingual corpus, where all the languages share both BPEed-token dictionary and transformer attention weights.
This deep transformer~\cite{vaswani2017attention} based pre-training model is expected to predict the correct text by seeing corrupted text. During this de-noising process, the model learns contextualized embedding for each token by conditioning on its long range neighboring tokens. Since transformer attention weights are shared across languages, common long range contextual information is learned during training.

% whay is it better
Our N-language pre-trained model can be used on all N*(N-1) language pairs and even on new pairs out of pre-training data. We also compare our pre-trained models with MASS~\cite{song2019mass}, where only 50\% masked tokens are predicted. Instead, we predict every token. In this way better decoder parameters can be learned during pre-training. Compared with other popular pre-train effort (eg: XLM~\cite{lample2019cross} initializing encoder and decoder separately and partially, our pre-training initialize all the parameters with one model. %Plus, we did a scale up on monolingual data corpus and number of languages. %as XLM-R~\cite{conneau2019unsupervised}.

% result
Then we select arbitrary pairs from the 25 languages used in pre-training and initialize a new seq2seq model with the pre-trained parameters. We are able to achieve remarkable results on low/medium resource supervised machine translation tasks. We  also include results and analysis on zero resource translation and document level machine translation tasks.

The finetuned models achieve significant gains (up to 12 BLEU points) across low/medium-resource pairs (<10M bi-text pairs), without sacrificing performance in high-resource settings. These results further improve with back-translation (BT), setting a new state-of-the-art on WMT16 English-Romanian and the FloRes test sets. For document-level MT, we obtain up to 5.5 BLEU improvements, without any task-specific modifications. For unsupervised MT, using a pre-trained seq2seq model allows us to significantly simplify model initialization.  Also, it produces the first non-degenerate results for less related language pairs (e.g., 9.5 BLEU gain on Nepali-English). We also demonstrate a new type of  unsupervised MT, where fine-tuning on bitext in one language pair (e.g., Korean-English) creates a model that can translate from all other languages in the monolingual pre-training set (e.g., Italian-English) with no further training. 

==> 03-data.tex <==
\section{Data}

\label{sec:data}
\subsection{Monolingual Datasets}
We use the same Common Crawl Corpus as that introduced in XLM-R~\cite{conneau2019unsupervised}. However, instead of using all 100 languages, we only select 25 languages among them, which have well established to English machine translation bi-text data and baselines. Table~\ref{tab:datastats} shows the sizes of monolingual corpora for these 25 languages that we use in our pretrainings. \input{Tables/languages.tex}
\subsection{Parallel Datasets}
In Table~\ref{tab:bitext} We show the bi-text amount in term of to English and resources for the 24 languages we choose. Most of pairs are from WMT and IWSLT. We also use FLoRes pairs~\cite{guzman-etal-2019-flores} (En-Ne and En-Si), En-Hi from IITB~\cite{DBLP:journals/corr/abs-1710-02855}, En-Ja~\cite{neubig11kftt}, and En-My from WAT19~\cite{chen2019facebook}. We divide those 24 language pairs into three categories -- row resource ( < 1M), medium resource ( < 10M and > 1M ), and high resource ( > 10M). 
\input{Tables/Bitex_stats.tex}
\subsection{Data Preprocessing}
We pre-processed the data with sentence piece model (SPM)~\cite{kudo-richardson-2018-sentencepiece}. We build the dictionary based on SPM on 100 languages which results in a  dictionary size of 250,000 BPEed tokens. All of our CC25, CC06, and bilingual models share the same dictionary (see section 4.1). \secomment{todo:Naman: add the up/down sampling tricks here.}

==> Tables/Bitex_stats.tex <==
\begin{table}[t]
\begin{center}
\small
\begin{tabular}{lrr}
\toprule
\bf Language pairs & \bf Bitext Size & \bf Data Source \\ 
%\midrule
%\multicolumn{3}{l}{\emph{Still Missing @Naman}} \\
%\textbf{En-Et} & & WMT18\\
%\textbf{En-Lv} & & WMT17\\
%\textbf{En-Kk} & & WMT19\\
%\textbf{En-Gu} & & WMT19\\
\midrule
\multicolumn{3}{l}{\emph{Low Resource Pairs}} \\
\textbf{En-Ro} & 608K & WMT16 \\
\textbf{En-Tr} & 207K & WMT17 \\
\textbf{En-Kk} & 91K & WMT19 \\
\textbf{En-Gu} & 10K & WMT19 \\
\textbf{En-My} & 259K & WAT19 \\
\textbf{En-Ja} & 440K & KFTT \\
\textbf{En-Ne} & 564K & FloRes\\
\textbf{En-Si} & 647K & FloRes\\
\textbf{En-Vi} & 133K & IWSLT15\\
\textbf{En-It} & 250K & IWSLT17 \\
\textbf{En-Nl} & 237K & IWSLT17\\
\textbf{En-Ar} & 250K & IWSLT17\\
\textbf{En-Ko} & 230K & IWSLT17\\
\textbf{De-Nl} & 214K & IWSLT17\\
\midrule
\multicolumn{3}{l}{\emph{Medium Resource Pairs}} \\
\textbf{En-Hi} & 1.56M & IITB\\
\textbf{En-Fi} & 2.66M & WMT17\\
\textbf{En-Lv} & 4.50M & WMT17\\
\textbf{En-Et} & 1.94M & WMT18\\
\textbf{En-Lt} & 2.11M & WMT19\\


\midrule
\multicolumn{3}{l}{\emph{High Resource Pairs}} \\
\textbf{En-Fr} & 41M & WMT14 \\
\textbf{En-Zh} & 25M & WMT17 \\
\textbf{En-Cs} & 11M & WMT18\\
\textbf{En-Ru} & 29M & WMT19 \\
\textbf{En-De} & 28M & WMT19 \\



\bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Bitext Statistics}
Bitext amount in terms of number of parallel sentence along with their source
}
\label{tab:bitext}
\end{table}

==> Tables/ne-en-transfer.tex <==
\begin{table*}[ht]
\begin{center}
\begin{tabular}{lccccccc}
\toprule

& \bf Nl-En & \bf Ro-En & \bf Cs-En & \bf Ar-En & \bf Ko-En & \bf Hi-En &  \bf Ne-En\\ 
& \multicolumn{7}{c}{\emph{Ne-En BLEU}}\\
\midrule
\textsc{\bf S2S}&0 &0&0&0&0&0&7.6\\

\textsc{\bf CC25}&3.0&4.3&5.0&5.2&6.5& 17.9&14.5 \\

\bottomrule

\end{tabular}
\end{center}
\caption{We test sacreble on Ne-En pair after fine tuned on Nl-En, Ro-En, Cs-En, Ar-En, Ko-En, Hi-En, and Ne-En (SupMT)}
\label{tab:ne-en-transferlearning}
\end{table*}
